Metal Lines Associated with the Lyman-alpha Forest from eBOSS Data

We investigate the metal species associated with the Ly$\alpha$ forest in the eBOSS quasar spectra. Metal absorption lines are revealed in the stacked spectra from cross-correlating the selected Ly$\alpha$ absorbers in the forest and the flux fluctuation field. Up to 13 metal species are identified associated with relatively strong Ly$\alpha$ absorbers (those with flux fluctuation $-1.0<\delta_{\rm Ly\alpha}<-0.6$ and with neutral hydrogen column density of ~ $10^{15-16}$ $\rm cm^{-2}$) over absorber redshift range of $2<z_{\rm abs}<4$. The column densities of these species decrease toward higher redshift and for weaker Ly$\alpha$ absorbers. From modelling the column densities of various species, we find that the column density pattern suggests contributions from multiple gas components both in the circumgalactic medium (CGM) and in the intergalactic medium (IGM). While the low-ionization species (e.g., C II, Si II, and Mg II) can be explained by high-density, cool gas ($T \sim 10^4$ K) from the CGM, the high-ionization species may reside in low-density or high-temperature gas in the IGM. The measurements provide inputs to model metal contamination in the Ly$\alpha$ forest baryon acoustic oscillations measurement. Comparison with metal absorptions in high-resolution quasar spectra and with hydrodynamic galaxy formation simulations can further elucidate the physical conditions of these Ly$\alpha$ absorbers.

==> authors.tex <==
\email{liyang@shao.ac.cn, zhengzheng@astro.utah.edu}

\author{Li Yang}
\affiliation{
Shanghai Astronomical Observatory, Chinese Academy of Sciences \\
80 Nandan Road, Shanghai 200030, People's Republic of China
}
\affiliation{
School of Astronomy and Space Sciences, University of Chinese Academy of Sciences \\
No.19A Yuquan Road, Beijing 100049, People’s Republic of China \\
}
\affiliation{
Department of Physics and Astronomy, University of Utah \\
115 S 1400 E, Salt Lake City, UT 84112, USA
}

\author{Zheng Zheng}
\affiliation{
Department of Physics and Astronomy, University of Utah \\
115 S 1400 E, Salt Lake City, UT 84112, USA
}

\author{H\'elion~du~Mas~des~Bourboux}
\affiliation{
Department of Physics and Astronomy, University of Utah \\
115 S 1400 E, Salt Lake City, UT 84112, USA
}

\author{Kyle Dawson}
\affiliation{
Department of Physics and Astronomy, University of Utah \\
115 S 1400 E, Salt Lake City, UT 84112, USA
}

\author{Matthew M. Pieri}
\affiliation{
Aix Marseille Universit\'e, CNRS, CNES, Laboratoire d’Astrophysique de Marseille \\
Marseille 13388, France
}

\author{Graziano Rossi}
\affiliation{
Department of Physics and Astronomy, Sejong University,\\
209, Neungdong-ro, Gwangjin-gu, Seoul, South Korea
}

\author{Donald P. Schneider}
\affiliation{
Institute for Gravitation and the Cosmos, Pennsylvania State University\\
University Park, PA 16802, USA
}
\affiliation{
Department of Astronomy and Astrophysics, Eberly College of Science, The Pennsylvania State University\\ 
525 Davey Laboratory, University Park, PA 16802, USA
}

\author{Axel de la Macorra}
\affiliation{
Instituto de F\'isica, Universidad Nacional Aut\'onoma de M\'exico, \\ 
Circuito de la Investigaci\'on Cient\'ifica Ciudad Universitaria, 04510  CDMX, M\'exico
}

==> tables.tex <==
%%% metal
%% tabel_Zabs2.1 tabel_Zabs2.3
\begin{table*}
\setcounter{table}{1}
\caption{Measurements of metal lines in the $2.0<\zabsorb<4.0$ stacked spectrum. Column density $N$ and Doppler parameter $b$ from Voigt profile fitting are in units of $\cm^{-2}$ and $\kms$, respectively.}
\label{table_Zabs[2.0,2.4]}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l*{14}{r}}
\hline
\hline
    \noalign{\smallskip}
Species & $\lambda$ (\AA) &  
\multicolumn{3}{c}{$-1.0\le \,$\dl$\, < -0.9$} &  
\multicolumn{3}{c}{$-0.9\le \,$\dl$\, < -0.8$}&  \multicolumn{3}{c}{$-0.8\le \,$\dl$\, < -0.7$}&  \multicolumn{3}{c}{$-0.7\le \,$\dl$\, < -0.6$} \\
& & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$}  & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} \\
\cutinhead{$2.0<\zabsorb<2.2$}
\input{table_Zabs2.1.txt}
\cutinhead{$2.2<\zabsorb<2.4$}
\input{table_Zabs2.3.txt}
    \noalign{\smallskip}
\hline
\end{tabular}
}
\end{table*}

%% tabel_Zabs2.5 tabel_Zabs2.7
\begin{table*}
\setcounter{table}{1}
\caption{(Continued)}
\label{table_Zabs[2.4,2.8]}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l*{14}{r}}
\hline
\hline
    \noalign{\smallskip}
Species & $\lambda$ (\AA) &  
\multicolumn{3}{c}{$-1.0\le \,$\dl$\, < -0.9$} &  
\multicolumn{3}{c}{$-0.9\le \,$\dl$\, < -0.8$}&  \multicolumn{3}{c}{$-0.8\le \,$\dl$\, < -0.7$}&  \multicolumn{3}{c}{$-0.7\le \,$\dl$\, < -0.6$} \\
& & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$}  & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} \\
\cutinhead{$2.4<\zabsorb<2.6$}
\input{table_Zabs2.5.txt}
\cutinhead{$2.6<\zabsorb<2.8$}
\input{table_Zabs2.7.txt}
    \noalign{\smallskip}
\hline
\end{tabular}
}
\end{table*}

%% tabel_Zabs2.9 tabel_Zabs3.1
\begin{table*}
\setcounter{table}{1}
\caption{(Continued)}
\label{table_Zabs[2.8,3.2]}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l*{14}{r}}
\hline
\hline
    \noalign{\smallskip}
Species & $\lambda$ (\AA) &  
\multicolumn{3}{c}{$-1.0\le \,$\dl$\, < -0.9$} &  
\multicolumn{3}{c}{$-0.9\le \,$\dl$\, < -0.8$}&  \multicolumn{3}{c}{$-0.8\le \,$\dl$\, < -0.7$}&  \multicolumn{3}{c}{$-0.7\le \,$\dl$\, < -0.6$} \\
& & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$}  & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} \\
\cutinhead{$2.8<\zabsorb<3.0$}
\input{table_Zabs2.9.txt}
\cutinhead{$3.0<\zabsorb<3.2$}
\input{table_Zabs3.1.txt}
    \noalign{\smallskip}
\hline
\end{tabular}
}
\end{table*}

%% tabel_Zabs3.1 tabel_Zabs3.5
\begin{table*}
\setcounter{table}{1}
\caption{(Continued)}
\label{table_Zabs[3.2,3.6]}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l*{14}{r}}
\hline
\hline
    \noalign{\smallskip}
Species & $\lambda$ (\AA) &  
\multicolumn{3}{c}{$-1.0\le \,$\dl$\, < -0.9$} &  
\multicolumn{3}{c}{$-0.9\le \,$\dl$\, < -0.8$}&  \multicolumn{3}{c}{$-0.8\le \,$\dl$\, < -0.7$}&  \multicolumn{3}{c}{$-0.7\le \,$\dl$\, < -0.6$} \\
& & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$}  & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} \\
\cutinhead{$3.2<\zabsorb<3.4$}
\input{table_Zabs3.3.txt}
\cutinhead{$3.4<\zabsorb<3.6$}
\input{table_Zabs3.5.txt}
    \noalign{\smallskip}
\hline
\end{tabular}
}
\end{table*}

%% tabel_Zabs3.7 tabel_Zabs3.9
\begin{table*}
\setcounter{table}{1}
\caption{(Continued)}
\label{table_Zabs[3.6,4.0]}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l*{14}{r}}
\hline
\hline
    \noalign{\smallskip}
Species & $\lambda$ (\AA) &  
\multicolumn{3}{c}{$-1.0\le \,$\dl$\, < -0.9$} &  
\multicolumn{3}{c}{$-0.9\le \,$\dl$\, < -0.8$}&  \multicolumn{3}{c}{$-0.8\le \,$\dl$\, < -0.7$}&  \multicolumn{3}{c}{$-0.7\le \,$\dl$\, < -0.6$} \\
& & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$}  & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} & \multicolumn{1}{c}{$\log N$}  & \multicolumn{1}{c}{$b$} & \multicolumn{1}{c}{$N_{pair}$} \\
    \cutinhead{ \tablecolumns{1}{$3.6<\zabsorb<3.8$}}
\input{table_Zabs3.7.txt}
\cutinhead{$3.8<\zabsorb<4.0$}
\input{table_Zabs3.9.txt}
    \noalign{\smallskip}
\hline
\end{tabular}
}
\end{table*}

==> thanks.tex <==
\begin{acknowledgements}
This work is supported by National Key R\&D Program of China (grant No. 2018YFA0404503).
L.Y. gratefully acknowledges the support of China Scholarship Council (No. 201804910563) and the hospitality of the Department of Physics and Astronomy at the University of Utah during her visit. Z.Z. is supported by NSF grant AST-2007499. The support and resources from the Center for High Performance Computing at the University of Utah are gratefully acknowledged. G.R. acknowledges support from the National Research Foundation of Korea (NRF) through Grant No. 2020R1A2C1005655 funded by the Korean Ministry of Education, Science and Technology (MoEST).

Funding for the Sloan Digital Sky 
Survey IV has been provided by the 
Alfred P. Sloan Foundation, the U.S. 
Department of Energy Office of 
Science, and the Participating 
Institutions. 

SDSS-IV acknowledges support and 
resources from the Center for High 
Performance Computing  at the 
University of Utah. The SDSS 
website is www.sdss.org.

SDSS-IV is managed by the 
Astrophysical Research Consortium 
for the Participating Institutions 
of the SDSS Collaboration including 
the Brazilian Participation Group, 
the Carnegie Institution for Science, 
Carnegie Mellon University, Center for 
Astrophysics | Harvard \& 
Smithsonian, the Chilean Participation 
Group, the French Participation Group, 
Instituto de Astrof\'isica de 
Canarias, The Johns Hopkins 
University, Kavli Institute for the 
Physics and Mathematics of the 
Universe (IPMU) / University of 
Tokyo, the Korean Participation Group, 
Lawrence Berkeley National Laboratory, 
Leibniz Institut f\"ur Astrophysik 
Potsdam (AIP),  Max-Planck-Institut 
f\"ur Astronomie (MPIA Heidelberg), 
Max-Planck-Institut f\"ur 
Astrophysik (MPA Garching), 
Max-Planck-Institut f\"ur 
Extraterrestrische Physik (MPE), 
National Astronomical Observatories of 
China, New Mexico State University, 
New York University, University of 
Notre Dame, Observat\'ario 
Nacional / MCTI, The Ohio State 
University, Pennsylvania State 
University, Shanghai 
Astronomical Observatory, United 
Kingdom Participation Group, 
Universidad Nacional Aut\'onoma 
de M\'exico, University of Arizona, 
University of Colorado Boulder, 
University of Oxford, University of 
Portsmouth, University of Utah, 
University of Virginia, University 
of Washington, University of 
Wisconsin, Vanderbilt University, 
and Yale University.

\end{acknowledgements}

